The Path Not Taken: RLVR Provably Learns Off the Principals

Reinforcement Learning with Verifiable Rewards (RLVR) reliably improves the reasoning performance of large language models, yet it appears to modify only a small fraction of parameters. We revisit this paradox and show that sparsity is a surface artifact of a model-conditioned optimization bias: for a fixed pretrained model, updates consistently localize to preferred parameter regions, highly consistent across runs and largely invariant to datasets and RL recipes. We mechanistically explain these dynamics with a Three-Gate Theory: Gate I (KL Anchor) imposes a KL-constrained update; Gate II (Model Geometry) steers the step off principal directions into low-curvature, spectrum-preserving subspaces; and Gate III (Precision) hides micro-updates in non-preferred regions, making the off-principal bias appear as sparsity. We then validate this theory and, for the first time, provide a parameter-level characterization of RLVR's learning dynamics: RLVR learns off principal directions in weight space, achieving gains via minimal spectral drift, reduced principal-subspace rotation, and off-principal update alignment. In contrast, SFT targets principal weights, distorts the spectrum, and even lags RLVR. Together, these results provide the first parameter-space account of RLVR's training dynamics, revealing clear regularities in how parameters evolve. Crucially, we show that RL operates in a distinct optimization regime from SFT, so directly adapting SFT-era parameter-efficient fine-tuning (PEFT) methods can be flawed, as evidenced by our case studies on advanced sparse fine-tuning and LoRA variants. We hope this work charts a path toward a white-box understanding of RLVR and the design of geometry-aware, RLVR-native learning algorithms, rather than repurposed SFT-era heuristics.

==> sections/2-pre.tex <==
\section{Related Works}
Move to later with related works
% \href{https://arxiv.org/pdf/2507.05386}{check}

\paragraph{RLVR}

\paragraph{Understanding of RLVR mechanisms}
A growing line of work probes RLVR’s mechanisms—asking whether RL chiefly \emph{discovers} new behaviors or \emph{sharpens} existing ones~\citep{liu2025prorl,wu2025invisible}, and whether it promotes \emph{generalization} or \emph{memorization}~\citep{chu2025sft,shenfeld2025rl}.
However, most analyses remain at an abstract level (e.g., policy KL or distributional drift~\citep{shenfeld2025rl}). 
This motivates a more mechanistic view: we peel back the layers to examine \emph{how} RL shapes model parameters and subspaces during training.

==> sections/3-method-3.tex <==
\section{Implication/other results of the three-gate model}
some implication, maybe focus on observation and explanation first, no need to put this as it will be too long for this paper

\hz{RL maybe too conservative from their base policy without the ability to touch the base knowledge, this confirms a mid-training or sft is required for those weaker foundation model like llama, while our analysis yields a more interesting perspective from which part of weights being touched}


\hz{low-entropy token is not purely not useful as it will also impact the internal dyanmics, while high-entropy token's grad seems only impact the final head layer, so recent papers doesn't drop those high-entropy tokens entirely while still keep low-etropy tokens but only assign more encouragement}


\paragraph{Dynamic sparse training helps perturb initial policy to a better point}

We indeed see better by just using random sparse training.

\paragraph{Another possible implication is for those self-rewarding RL such as \href{Co-rewarding}{https://github.com/tmlr-group/Co-rewarding}, using the lowest magnitude mask can cover with a ratio $>95\%$.}
I guess pure based on model self-reward, they follow more coherently with the optimization bias


\iffalse
\subsection{Dynamic Sparse Warm-Start (DSW)}
\label{sec:dsw}

We insert a short, randomized sparse phase at the start of RL: we mask a fixed fraction of
coordinates \emph{before} clipping and optimizer updates, refresh the mask every $T$ steps,
and release all coordinates after $K_{\mathrm{free}}$ steps (then train dense as usual).
Let $q\in(0,1]$ be the keep-rate (we use $q=0.5$).

\paragraph{Where the mask acts.}
For a linear projection with pre-clip gradient $G=\delta h^\top$ (eqs.\,(C1)–(C2)),
we apply an entrywise Bernoulli mask $M\in\{0,1\}^{m\times n}$ to obtain
$\tilde G = M\odot G$ \emph{before} computing the layer/group clip factor; then
\[
\tilde\alpha \;=\; \min\!\left(1,\;\frac{\tau}{\|\tilde G\|_F}\right),\qquad
\Delta W \;=\; -\eta\,\tilde\alpha\,\big(P_{\mathrm{opt}}\odot \tilde G\big),
\]
as in (C2). We refresh $M$ every $T$ steps and set $M=\mathbf{1}$ after $K_{\mathrm{free}}$ steps.

\begin{algorithm}[H]
\caption{Dynamic Sparse Warm-Start (DSW) for one layer}
\label{alg:dsw}
\begin{algorithmic}[1]
\REQUIRE keep-rate $q$, refresh period $T$, release step $K_{\mathrm{free}}$, clip $\tau$
\FOR{training step $k=1,2,\dots$}
  \STATE form pre-clip gradient $G_k=\delta_k h_k^\top$ \hfill (eq.\,(C1))
  \IF{$k\le K_{\mathrm{free}}$}
    \IF{$k \bmod T = 1$} \STATE sample $M_k \sim \mathrm{Bernoulli}(q)$ entrywise \ENDIF
    \STATE $\tilde G_k = M_k \odot G_k$
  \ELSE
    \STATE $\tilde G_k = G_k$ \hfill (dense phase)
  \ENDIF
  \STATE $\tilde\alpha_k = \min\!\left(1,\;\frac{\tau}{\|\tilde G_k\|_F}\right)$ \hfill (eq.\,(C2))
  \STATE $\Delta W_k = -\eta\,\tilde\alpha_k\,\big(P_{\mathrm{opt}}\odot \tilde G_k\big)$
  \STATE $W \leftarrow W + \Delta W_k$
\ENDFOR
\end{algorithmic}
\end{algorithm}

\paragraph{Why DSW works under the Three-Gate view.}
Masking \emph{before} clipping reduces the gradient norm seen by the clip, so
$\tilde\alpha$ increases and the per-active-entry update is amplified, helping more
coordinates cross the bf16 gate (Gate~III), while the layer-level trust region remains intact.

\begin{lemma}[Budget concentration under clipping]
\label{lem:dsw}
Assume clipping is active in a layer, i.e., $\alpha=\tau/\|G\|_F < 1$ in (C2).
With an i.i.d.\ Bernoulli mask of keep-rate $q$, we have
$\mathbb{E}\|\tilde G\|_F^2 = q\|G\|_F^2$ and $\mathbb{E}\tilde\alpha \approx \alpha/\sqrt{q}$.
Consequently, for any unmasked entry $(i,j)$,
\[
\mathbb{E}\big[|\Delta W_{ij}|\;\big|\;M_{ij}=1\big]\;\approx\;
\frac{1}{\sqrt{q}}\cdot \eta\,\alpha\,p_{ij}\,|G_{ij}|
\]
while the layer-level step remains bounded by $\tau$ (trust region).
\end{lemma}

\noindent
By Lemma~\ref{lem:dsw} and the bf16 gate (C3)–(C6), concentrating the per-entry step
increases the chance that $|\Delta W_{ij}| \gtrsim \tfrac12\,\mathrm{ulp}_{\text{bf16}}(W_{ij})$,
leading to higher coverage of \emph{realized} changes at the same KL budget (Gate~III).
Randomizing the mask every $T$ steps perturbs the inherited routing (Gate~II), so the
trajectory explores a union of low-curvature subspaces before converging in the dense phase.
\fi
